Semantic of Cloud Computing services for Time Series workflows

Time series (TS) are present in many fields of knowledge, research, and engineering. The processing and analysis of TS are essential in order to extract knowledge from the data and to tackle forecasting or predictive maintenance tasks among others The modeling of TS is a challenging task, requiring high statistical expertise as well as outstanding knowledge about the application of Data Mining(DM) and Machine Learning (ML) methods. The overall work with TS is not limited to the linear application of several techniques, but is composed of an open workflow of methods and tests. These workflow, developed mainly on programming languages, are complicated to execute and run effectively on different systems, including Cloud Computing (CC) environments. The adoption of CC can facilitate the integration and portability of services allowing to adopt solutions towards services Internet Technologies (IT) industrialization. The definition and description of workflow services for TS open up a new set of possibilities regarding the reduction of complexity in the deployment of this type of issues in CC environments. In this sense, we have designed an effective proposal based on semantic modeling (or vocabulary) that provides the full description of workflow for Time Series modeling as a CC service. Our proposal includes a broad spectrum of the most extended operations, accommodating any workflow applied to classification, regression, or clustering problems for Time Series, as well as including evaluation measures, information, tests, or machine learning algorithms among others.

==> Time Series Workflow for CC-1/abstract.tex <==
%
% REVISAR.

Time series (\TS{}) are present in many fields of knowledge, research, and engineering. The processing and analysis of \TS{} are essential in order to extract knowledge from the data and to tackle forecasting or predictive maintenance tasks among others The modeling of \TS{} is a challenging task, requiring high statistical expertise as well as outstanding knowledge about the application of Data Mining (\DM{}) and Machine Learning (\ML{}) methods. The overall work with \TS{} is not limited to the linear application of several techniques, but is composed of an open \WFlong{} of methods and tests.
These \WFlong{}, developed mainly on programming languages, are complicated to execute and run effectively on different systems, including Cloud Computing (\CC{}) environments. The adoption of \CC{} can facilitate the integration and portability of services allowing to adopt solutions towards services Internet Technologies (\IT{}) industrialization. The definition and description of \WFlong{} services for \TS{} open  up a new set of possibilities regarding the reduction of complexity in the deployment of this type of issues in 
\CC{} environments. In this sense, we have designed an effective proposal based on semantic modeling (or vocabulary)  that provides the full description of  \WFlong{} for \TSlong{} modeling as a \CC{} service. Our proposal includes a broad spectrum of the most extended operations, accommodating any \WFlong{} applied to classification, regression, or clustering problems for \TSlong{}, as well as including evaluation measures, information, tests, or machine learning algorithms among others. 


% Abstract - RE-DONE
% --------------------
% Que son las TSy para que son importantes
% Como se hace en anñalisis actual y 
% que problema tiene este analysis y trabajo tradicional con TS. 
% Flujo de trabajo de TS en Cloud Computing y sus ventajas.
% Propuesta.



==> Time Series Workflow for CC-1/conclusions.tex <==
 \section{Conclusions and future work}
 \label{sec:conclusions}
 
 %% En este artículo hemos presentado un esquema para la descripción 
 %% de servcios y flujos de trabajo para CC específicamnete diseñados para 
 %% el procesamiento y analiss de series temporales llamado tswf-scjhema. 
 %% El esquema que se ha desarrollado aglutina toda la operativa 
 %% comumnente tutilizada en el estudio y analisis de series temporales, 
 %% lo que permite transformar cualquier implementación ya 
 %% desarrollada en otros lenguajes como R o Python en una implementación 
 %% basada en tecnología semántica mucho más rica, homogénea y fácilmente portable. Esta portabilidad es clave 
 %% en cuanto a que una única definición de un flujo de trabajo con tswf-schema sería 
 %% gestionable y desplegable en cualquier proveedor de servicios de cloud, 
 %% facilitando enormemente la industrialización de servicios en CC. Con el esquema desarrolado junto con otros esquemas tales como dmcc-schema se tiene la posiblidad de incluir en la definición de un servicio o flujo de traajo con series temporales todos los elementos relativos a la gestión de un servicio de CC como precios, SLA o catalogos de proveeedores, aprovenchando las directivas de Linked Data.
 
 %% Los casos de uso seleccionados permiten por un lado mostrar al usuario que cualquier implementación de flujo de trabajo puede ser transformada en una especificación semántica con twsf-schema lista para ser condumida en entornos Cloud Computing, y por otro lado pone en valor la necesidad de poseer una homegenizaciuón en la definición de servicios de computación de este tipo, que por desgracia  el mercado de proveedores de servicios acualmente carece. Además, gracias a las CQ es posible responder a un subconjunto de características deseables  que un ingenierio de servicios en Cloud COmputkng podría necesitar. Tanto la efectivdad como la eficaica han sido destacadas en esta validación de los casos de uso.
 
 %Finalmente como trabajo futuro proponemos la implementación de un Broker de servicios de Cloud Computin para TS que tenga la capacidad  de optimizar un flujo de trabajo escrito en tswf-schema aprovechando las  implemntaciones de algorimos y la capacidad de computación sobre diferentes plataformas de CC. 
 
 
 In this article we have introduced a scheme for the description of services in \CC{} specifically designed for \TS{} processing named \tswfschema{}.  The scheme developed brings together all the commonly used operations in the study and analysis of \TS{}, which allows transforming any implementation already developed in languages such as \textit{R} or \textit{Python} into  a description based on semantic technology much richer, more homogeneous, and portable. This portability is key in terms of the fact that a single definition of a workflow with \tswfschema{} would be manageable and deployable in any \CC{} service provider significantly facilitating the industrialization of services for \CC{} environments.
 
 With the scheme developed together with other complementary ones such as \texttt{dmcc-schema}, it is possible to include in the definition \TS{} workflow all the elements related to the management of a \CC{} service such as prices, SLA or instances, among other, taking advantage of the \textit{Linked Data} proposal.  
 
 The selected use cases allow, on one hand, to show the user that any workflow implementation can be transformed into a semantic specification with \tswfschema{} ready to be consumed in \CC{} environments, and on the other hand, it highlights the need to have a homogenization in the definition of this type of computing services, which unfortunately the \CC{} service providers market lacks. In addition, thanks to CQs it is possible to respond to a subset of desirable features that a service engineer in Cloud Computing might need. Both effectiveness and efficiency have been highlighted in the uses case validation.  
 
 Finally, as a future work, we propose the implementation of a Cloud Computing services broker for \TS{} that has the ability to optimize a workflow written in \tswfschema{} taking advantage of algorithm implementations and computing capabilities over different \CC{} platforms. 

==> Time Series Workflow for CC-1/introduction.tex <==

% Prediccion de acciones en la bolsa, estimacion de la produccion y consumo de productos o forecasting de la temperatura y precipitaciones de un lugar, son entre muchas,  actividades de analisis de datos donde se prima el estudio de  series temporales como  componentes fundamentales para el exito del modelado en predicción.En el momento actual donde la computación en la nube prácticamente se ha integrado de una manera totalmente transparente en nuestras relacion con las tecnologías de la información e Internet, las actividades relacionadas con el análisis de datos en general y de forma aún sostenida,  con la predicción de series temporales, que avanza cada vez más  dentro del espectro de servicios ofertados por las plataformas de servicios en Cloud Computing.

\IEEEPARstart{F}{orecasting}  of weather conditions, the estimation of the value of stock market shares, or the detection of anomalies on industrial processes among others, are part of the set fields where the \TS{} data analysis plays a basic role to tackle knowledge extraction.

%Las series temporales son una secuencia o secuencias de datos espaciados en el tiempo; eventos, actividades o dispositivos generan continuamente información que se marca temporalmente y se almacena para estudio en tiempo real o posprocesado. De forma creciente en interes, el uso de dispositivos, las actividades de usuarios, vehiculos, agricultura, autómatas, o la llamada IoT entre otros, producirán una ingente cantidad de información en los proximos años y un importante porcenataje de esa información será en forma de Series temporales. No solo en volumen de datos, si no en cantidad de negocio, en concreto según Ericcsson en su informe [REF], el flujo de información que se moverá supondrá en torno a los 69Bn dólares para los próximos años. Estas cifras dan información de sobra de la necesidad de procesamiento de este tipo de datos. Las series temporales, necesitarán ser procesados en forma de servicios de computación en la nube siguiendo las características fundamentales  de flexibilidad, escalabilidad y seguridad defindas por el NIST.

Time series is a sequence or sequences of data spaced out in time; events, activities, or devices continuously generate information that is temporarily logged and stored for real-time or post-processed study. The work with \TS{} is one of the fastest growing at the moment, due to the proliferation of the so-called IoT \cite{gubbi2013internet},  for instance.  Increasingly in interest, the use of mobile devices, autonomous vehicles, modern agriculture, or intelligent machines, will produce a huge amount of information in the coming years and a significant percentage of this information will be in the form of \TS{} data \cite{ericsson2018}. 
%According to Ericsson in his report , the amount of information that will be moved will be around 69 Bn dollars for the next few years. 

At the present time, when \CC{} has practically been integrated in a totally transparent way in our relationship with Information Technologies (IT) and Internet, the activities related to data analysis are incrementally being added to the spectrum of services offered by the \CC{} platforms and providers. Analysis and study of \TS{}  will need to be processed as \CC{} services following the NIST\cite{mell2011nist} recommendations such as flexibility, scalability, portability, and security.



%El auge de la computación en la nube en paralelo con el aumento de la capacidad de cálculo de computación ha favorecido la implantación de herramientas y plataformas para el analisis  y la minería de datos. Estás herramientas  y frameworks proveen de un amplio abanico de métodos, funciones y algoritmos para realizar el procesamiento de los datos en todas las escalas, tanto desde escritorio[REFs],  grandes clusters[REFs] o bien desde plataformas de servicios en CC.

The rise of \CC{} in parallel with the increase in computing  capability has led to the deployment of tools and platforms for data mining and data analysis. Both offer  a wide range of methods, functions and algorithms to perform data processing at all scales, either from the desktop \cite{hall2009weka}, \cite{witten2016data}, large clusters \cite{zikopoulos2011understanding}, \cite{meng2016mllib}, \cite{mckinney2010data} or from service platforms in \CC{} \cite{hashem2015rise}.

%Estos proveedores de cloud computing ofrecen sus entornos de trabajo y servicios totalmente transparentes a los usuarios, proveyendoles de herramientas muy potentes para el análisis y la extracción de información de los datos junto con la aplicación de técnicas de Inteligencia Artificial. Dentro del área de la minería de datos, estos proveedores y plataformas cloud, no ofrecen apenas funcionalidades de servicios de Series Temporales dentro de su catalogo de servicios en CC. Esto supone tener que implementar en cada una de las plataformas provistas por los proveedores de servicios los métodos y algortimos especificos para el trabajo con series temporales. Además, el modelado de series temporales puede ser una tarea de análisis no lineal y de elevada complejidad. En el estudio del modelado de series temporales intervienen diferentes estudios o metodologías, compendios de aplicación de técnicas de DMML, modelos, o distintas valoraciones de medidas de rendimiento o precisión en los resultados, entre otros. El flujo de trabajo con series temporales puede ser realmente complejo si además este se necesita  implementar desde un servicio para cloud computing.


%\CC{} providers offer environments and services, adding powerful tools for the analysis and extraction of knowledge with the application of Artificial Intelligence (AI) and \ML{} techniques.

Within the area of \DM{}, these \CC{} providers and platforms offer barely \TS{} services and methods in a catalog of services \cite{hashem2015rise}. This means having to implement specific methods and algorithms for working with \TS{} on each provider platform or to migrate all the source code developed in a specific programming language and to ensure the entire service deployment will work properly. \TS{} modeling can be a highly complex and it supposes a non-linear analysis tasks \cite{hamilton1994time} including  a set of methods of the application of \DM{} and \ML{} techniques \cite{harris2003applied},  models, evaluations of performance or precision measurements, among other, that can be seen as a workflow of tasks.

%Time series \WFlong{} can be really complex when it is implement on a cloud computing service.



% 
%Gran parte de la problematica que ofrecen los servicios de cloud, proviene de la falta de integración con distintas plataformas de computacion en la nube. A la hora de la  migración de servicios  de un proveedor a otro lo ideal sería  una acosejable estandarización  de la descripción de servicios relacionados con Series temporales en CC. ...

The services of \TS{} analysis along \CC{} service providers address a lack of integration from heterogeneous and non-standardized cloud computing platforms. When migrating services from one \CC{} provider to another, the ideal solution would be to harmonized the description of services and \WFlong{} related to \TS{} on \CC{} deployments, abstracting the programming language or the architecture of deployment. This would allow the interoperability of these services between providers to be exploited more efficiently and offer all the scalability and flexibility advantages provided by the \CC{} paradigm. With this idea we pursue the industrialization of IT services through pre-designed and pre-configured solutions that are highly automated and repeatable, scalable and reliable, by meeting the needs of users or organizations.



%En este trabajo proponemos una definición de servicios para flujos de trabajo complejos con Series Temporales sobre plataformas CC.   La definición de los servicios se ha implementado siguiendo la propuesta de Linked Data. Para ello no solo se han implementado un extenso espectro de funciones y algoritmos relacionados con el Series Temporales, si no que tambiíen se ha trazado el modelado de fujo de tranbajo de las Series Temporales. Para la descripción de los diferenres componentes, se han usado vocabularios y esquemas ya exintes, completando al descripciíjn global de este tipo de servicio. Nosotros presentamos la propuesta tswf-schema, una propuesta de definición de flujo de trabajo y modelado de ST, que junto con dmml-schema, permiten cubir la deifnición completa de servicois en cloud. Además se ha desarrollado el middlewre que transforma la definición del flujo de modelado de ST en los algoritmos concretos ejecutables sobre la infraestructura.

The aim of this paper is to propose a definition of services for \TS{} \WFlong{} in \CC{}  environments based on semantic technology, % and by the other hand to develop a platform of proof-of-concept to validate the deployment of the \TS{} services proposed. The definition of services has been 
according to the Linked Data \cite{bizer2011linked} proposal. To address this definition, an exhaustive set of functions and algorithms related to the \TS{} and the \WFlong{} modeling have been specified and implemented (such as data pre-processing, visualization, modeling, or precision measures, among other). For the description of the different components and structures, existing service description schemes \cite{vandenbussche2017linked} have been re-used, improving the overall comprehension of the services. As a result, the \tswfschema{} proposal has been developed, a \WFlong{} definition and \TS{}  modelling, which together with \textit{dmcc-schema} \cite{parra2018data} allow to cover the complete definition of \CC{} services for \WFlong{}. 

%In addition, middleware has been developed that transforms the definition \TS{} \WFlong{} services into a concrete web service that can be executed on \CC{} infrastructures.



% Este trabajo se encuentra estructura del sigueinte modo: En la siguiente sección (X), presentamos los trabajos relacionados dentro del ambito de series temporales como su modelado y análisis, flujos de trabajo de minería de datos o aspectos de ST y CC. Section (Y) presenta la propuesta de definición de servicio CC de TS para WF, incluyendo cada uno de los elementos considerados para el modelado de ST, tales como analisis de estacionalidad, métodos de predicción o preprocesamiento entre otros. En la sección (Z), describimos la implementación del middleware que interconecta la definicón con la infraestructura y algunos resultados de las pruebas con ejemplos reales. Varios casos de uso son implementados desde la  desfinicio  de servicio para FWF en ST desde el libro de Hyndman [REF]. Por último las conclusiones de trbajo y las propuestas de trabajo futuro son expuestas en la sección G.

This paper is organized as follow: in the next section (\ref{sec:relatedwork}), we present the related work within the scope of \TS{} such as its modelling and analysis, data mining \WFlong{} and aspects of \TS{} and \CC{}. Section \ref{sec:timeseries}  presents the proposed \CC{} service definition of \TS{} for \WFlong{}, including each of the elements considered for \TS{} modelling, such as seasonality analysis, prediction methods or pre-processing, among others. In the section \ref{sec:usecases}, %we describe the implementation of the middleware that interconnects the definition of the services  with the infrastructure and test results with real examples. S
several use cases are implemented. Finally, the conclusions of the work and the proposals for future work are set out in section \ref{sec:conclusions}.



==> Time Series Workflow for CC-1/relatedworks.tex <==
\section{Related Work}
\label{sec:relatedwork}



% El análisis de series temporales es un tópico muy estudiado en la literatura científica, abordado desde distintas perspectivas y aplicado a multiples campos del conocimiento. El modelado de series temporales es una área muy dinámica que está atrayendo el interés de la comunidad científica cada vez más.  En el modelad de series temporales se busca estudiar de manera concienzuda los datos de las observaciones pasadas de la serie temporal en orden de crear un modelo que describa la serie temporales al completo, dentro de unos intervalos mínimos de fiabilidad. Parte importante del trabajo realizado con series temporales se ha desarrollado dentro de temáticas muy variadas tales como negocios, economía, acciones, ciencias ambientales o ingeniería entre otros [REFS].


\TSlong{} analysis and modeling is a very dynamic area that is attracting the interest of the scientific community in an incremental manner, due to the rise of IoT environments and knowledge extraction from  data sources in real time or offline. In this way, an important part of the work carried out with time series has been developed within distinct fields such as business, economics, stock market, environmental sciences, industrial monitoring, or engineering among others \cite{dominici2002use, aljawarneh2016similarity, xu2014tsaaas}.

%El análisis y modelado de ST es una tarea compleja  que incluye la  aplicación de diversas operaciones, técnicas y algoritmos. Este procedimiento puede verse como un flujo de trabajo que tiene como objetivo la resolución de problemas con datos de TS. 

The analysis and modeling of \TS{} is a complex task that includes the application of various operations, techniques and algorithms. This procedure can be seen as a \WFlong{}, covering a large number of methods and techniques to apply and focused on solving \TS{} problems \cite{montgomery2015introduction}.

% El análisis de las series temporales ha sido estudiado en profundidad y no hay un criterio único que establezca cual es el procedimiento a realizar para el flujo de trabajo en este tipo de problemas. Existen diversas metodologías para abortar el problema del modelado y la aproximación a la resolución de TS. La propuesta más ampliamente usada es la metodología Box-Jenkins. Esta metodología puede ser considerada como un flujo de trabajo no lineal. Box-Jenkins es utilizada en el proceso de construcción del modelo ARIMA para la ST abarcando aspectos como identificación, estimación, test y aplicación de métodos. Si nos centramos en el modelado, técnicas emparentadas con ARIMA, tales como AR, MA o ARMA, son también utilizandos como parte del proceso de flujo de trabajo con TS. El modelado de TS desde una perspectiva no-lineal ha sido abordado con el uso de ANN, bi-linear model, TAR o ARCH. Otras técnicas de modelado basadas en Minería de datos y Machine Learning han sido propuestas incluyendo RF, SVM, NN, o las más modernas como DeepLearn. En el análisis de TS se incluyen además, un amplio conjunto de tareas de procesamiento de datos ETL.

The analysis of the time series has been studied in depth and there is no single criterion that establishes which is the procedure to be carried out for the \WFlong{} in this type of problem. There are different methodologies to tackle the problem of modelling and the approach to \TS{} resolution. The most widely used proposal is the Box-Jenkins methodology \cite{tang1991time}. This methodology can be considered as linear \WFlong{}. Box-Jenkins is used in the construction process of the ARIMA \cite{chatfield2016analysis} model for the \TS{} covering aspects such as identification, estimation, error-testing and application of methods and modelling \cite{makridakis1997arma}. Focusing  on modelling, techniques related to ARIMA, such as AR, MA or ARMA \cite{ubeyli2004spectral}, are also used as part of the \TS{} \WFlong{} process. The modelling of \TS{} from a non-linear perspective has been approached with the use of ANN \cite{zhang2003time}, bi-linear model, TAR or ARCH \cite{engle2001garch}. Other modelling techniques based on \DM{} and \ML{} have been proposed including \RFlong{} \cite{liaw2002classification}, \SVMlong{} \cite{hearst1998support}, \NNlong{} \cite{zhang2003time}, or the more modern \DLlong{} one as in \cite{yang2015deep}. The \TS{} analysis also includes a comprehensive set of \ETLlong{} (ETL) data processing tasks \cite{hoey2014system}.



% Para la resolución de este tipo de análisis comunmente se han usado lenguajes y herramientas de programación, además de plataformas de minería de datos. Estas utilidades incluyen todo lo necesario en cuanto a componentes y funciones para el flujo de trabajo relativo TS. Lenguajes como R (con su taskview para TS) o Python (librerias especificas para TS),  paquetes de software como SAS o MathLab y entornos de minería de datos como KNIME, WEKA o UGRPlat, ofrecen las herramientas para hacer efectivo el trabajo con TS. En todas ellas es posible diseñar un flujo de trabajo con TS donde se puede concretar la aplicación de operaciones, visualizar los resultados, validar errores y aplicar multiples algoritmos para el modelado y posterior predicción.

\textcolor{red}{TODO: add missing [REF] and figures  in the document}
For the resolution of this type of analysis, programming languages and tools have been widely used, in addition to \DM{} platforms \cite{jovic2014overview}. These utilities include all the required components and functions for the relative \TS{} \WFlong{}.  Languages such as R (with its task-view for TS) \cite{hothorn2018cran} or Python (TS-specific libraries) \cite{vanderplas2016gatspy}, software packages such as SAS [REF] or MathLab [REF] and \DM{} environments such as KNIME \cite{berthold2009knime} or WEKA \cite{hall2009weka}, offer the tools to make effective the work with \TS{}. In all of them, it is possible to design a \WFlong{} where you can specify the application of operations, visualize the results, validate errors and apply multiple algorithms for the modelling and subsequent forecasting, classification or clustering \cite{rangra2014comparative}. 



% La mayor parte de las herramientas tradicionales  de análisis de series temporales están diseñadas para trabajar computadores de escritorio y no están preparadas para ser usadas en entornos de computación en la nube. Aprovechando las capacidades de computo de organizaciónes, parte de esa basto conjunto de recursos e infraestrctura están siendo destinados a Minería de datos y machine learning como servicios de CC bajo demanda. El análisis de series temporales no es una excepticón y  cada vez más los proveedores de cloud están incluyendo dentro del catalogo de servicios funciones y algoritmos específicos para el trabajo con Series Temporales. Actualmente hay una  demanda creciente de servicios que permitan desplegar un flujo de trabajo completo sobre un conjunto de datos tales como ST. Estos fujos de trabajo sonre problemlas de DM/ML sobre cloud son muy interesantes debido a su caracter escalable. Existe una clara necesidadad de mover gran parte del procesamiento de datos a plataformas en la nube, abstrayendo la infraestuctura de computación subyacente y las necesidades de escalado, ambas asegurdaras. 


Most traditional time series analysis tools are designed to work with desktop computers and are not ready to be used in \CC{} environments. Leveraging the computing capabilities of organizations, part of that vast set of resources and infrastructure are being allocated to \DM{} and \ML{} as on-demand \CC{} services \cite{hashem2015rise}. \TS{}  analysis is no exception and more and more \CC{} providers are including specific functions and algorithms for working with \TS{} services in their catalog \cite{chen2015data}. Currently, there is a growing demand for services that allow creating   \WFlong{} to be deployed over \CC{}, such as \TS{} \cite{marozzo2016workflow,chen2014big}. These \WFlong{} are very interesting because of their scalable character existing a clear need to move much of the data processing to cloud platforms, abstracting the underlying computing infrastructure and scalability needs, both of which will be assured \cite{kranjc2015active,kranjc2012clowdflows}. 

% Uno de los principales problemas de los servicios de CC es la falta de una definicion más o menos estandarízada de ests servicios entre los diferentes proveedores. Esto ocurre de igual modo con la descripcion de flujos de trabajo y  experimentación con datos en CC en el analisis de Series Temporales. La portabilidad de servicios y la capacidad de abstraer la infraestructura subyacente hace necesario el estudio de este tipo de problemáticas sobre CC.

One of the main problems of \CC{} services is the lack of a consistent and standardized definition of these services among the different \CC{} providers and it has been widely studied  \cite{dillon2010cloud, barry2003web}. This happens in the same way with the description of  \WFlong{} and experimentation with data in \CC{} in the analysis of \TS{}. The portability of services and the ability to abstract the underlying infrastructure makes it necessary to validate this type of problem on \CC{} platforms \cite{fox2009above} .

\WFlong{} modeling for \DM{} experimentation is considered in \cite{talia2013clouds}, \cite{data2013cloud} performing \WFlong{} as \CC{} services giving the user the ability to deploy a work of experimentation in an integral way. Several approaches manage the problem of the description of \WFlong{} dealing with ontology-based such us RDF or Turtle \cite{world2014rdf}. Those languages for \WFlong{} definition have been discussed in \cite{youseff2008toward} and \cite{iosup2011performance}. 

The definition and description of generic  \CC{} services that integrate multiple aspects of experimental work for \DM{} have been worked from the scope of the Linked Data \cite{bizer2011linked} proposal. Research papers such as DMOP \cite{keet2014exploring}, Exposé \cite{panov2014ontology}, dmcc \cite{parra2018data}  or MLSchema \cite{esteves2016ml} are examples of languages proposals for the definition of generic data mining services and \WFlong{}, related to \ML{}. These provide an adequate definition of services using a highly flexible definition language and linked to the natural development of the \CC{}.

Most of the proposals allow the development of experimental analysis, including part of the usual \WFlong{} with data processing and algorithms \cite{vockler2011experiences}. In these works the \WFlong{} modeling with \TS{}  is not taken into account being a fundamental element for the integration of these services within \CC{} platforms \cite{khan2012workload}. These types of problems need to bring together the different techniques and algorithms of \TS{} modeling, pre-processing \cite{garcia2015data}, performance measurements [REF], visualization [REF], or predictive models among others. In our work, a proposal of \WFlong{} modeling for \TS{} in \CC{} has been developed, which allows to tackle the work with the \TS{} experimentation and modeling using Linked Data recommendation on services description in  \CC{} platforms.


%The analysis of time series is a topic widely studied in the scientific literature, approached from different perspectives and applied to multiple fields of knowledge. , within minimum intervals of reliability. .


%Una propuesta ampliamente utilizada es conocida como la metodologías Box-Jenkins, utilizada en proceso de construcción del modelo de la ST en ARIMA. En Box-Jenkins se sigue una metodología tal que distingue diferentes fases, como identificación, Estimación o tests y Aplicación [REF:"ARMA Models and the Box-Jenkins Methodology (Journal of Forecasting) with M. Hibon.pdf"] y desde donde en cada fase realiza diferentes operaciones.

%A widely used approach is known as the Box-Jenkins \cite{tang1991time} methodology, used in the process of building the ST model at ARIMA \cite{chatfield2016analysis}. Box-Jenkins follows a methodology that distinguishes different phases, such as identification, estimation or tests and application \cite{makridakis1997arma} and from where each phase performs different operations.

%[REF: "ARMA Models and the Box-Jenkins Methodology (Journal of Forecasting) with M. Hibon.pdf"] 


%La predicción de series temporales ha sido tratado en profundidad desde diferentes perspectivas lineales estadísticas. ARIMA es el más utilizado para el modelado de series temporales, así como sus variantes AR ,MA, o ARMA. Al igual que para perspectiva lineal, el problema del modelado de ST, se ha tratado desde modelos no lineales tales como las ANN [REF:10.1.1.462.3756.pdf] al igual que con otros como como el bi-linear model, TAR, o ARCH modelo. 

%The prediction of time series has been treated in depth from different statistical linear perspectives. ARIMA is the most commonly used for time series modeling, as well as its AR ,MA, or ARMA variants \cite{ubeyli2004spectral}. As for linear perspective, the problem of ST modeling has been addressed from non-linear models such as the ANN \cite{zhang2003time} as well as others such as the bi-linear model, TAR, or ARCH model \cite{engle2001garch}.

%No sólo estos modelos han sido utilizados, también se han considerado diferentes algoritmos del área de la minería de datos e inteligencia artificial. Entre estos podemos citar aquellos más en auge como RANDOM [REF], FOREST, SVM [REF], NN [REFs] o los actuales basados en DEEPLearn [REFs].

%Not only have these models been used, but also different algorithms from the area of data mining and artificial intelligence have been considered in order to solve or approximate the problem of analysis and forecasting. Among these we can mention the most popular ones such as Random Forest \cite{liaw2002classification},  SVM \cite{hearst1998support} or the current ones based on Deep Learning \cite{yang2015deep}.


%El análisis y procesado de ST sobre plataformas CC se ha tratado en los trabajos científicos propuestos en X, Y.

%The analysis and processing of ST on CC platforms has been addressed in the proposed scientific papers in X, Y.


%Con el incremento de la capacidad de computo disponible y la necesidad de procesar grandes cantidades de datos de forma distribuida, la aplicación de técnicas de minería de datos y machine learning dentro de plataformas cloud computing ha sido tratado en muchos trabajos de investigación en los últimos años. No sólo el análisis de esos datos, sino también el flujo de trabajo y la gestión del mismo dentro de las  plataformas de cloud computing, está teniendo gran demanda de trabajos de investigación recientemente. En [REF:marozzo2016workflow]  y [REF:liu2014survey] se trata gran parte de la problemática sobre fujo de trabaojo en CC. Trabajos como [REF:zhang2015cloudflow], [REF:kranjc2015active], [REF:kranjc2012clowdflows], [REF:mierswa2006yale] proponen herramientas en CC para la gestión de los flujos de trabajo en CC. 

%With the increase in available computing capacity and the need to process large amounts of data in a distributed manner, the application of data mining and machine learning techniques within cloud computing platforms has been addressed in many research papers in recent years. Not only the analysis of this data, but also the workflow and management of it within the cloud computing platforms, has recently been in great demand for work. In \cite{marozzo2016workflow} and \cite{chen2014big}, a large part of the problem of workflow in CC is dealt with. Research works such as \cite{zhang2015cloudflow}, \cite{kranjc2015active}, \cite{kranjc2012clowdflows}, \cite{mierswa2006yale} offer CC tools and frameworks in order to manage general CC workflows.


%Aplicaciones para el análisis y modelado de TS se han desarrollado en GHZ. Dentro dl campo de la computación en la nube y la aplicación  de técnicas y algoritmos para a la resolución de TS  hay que considerar los siguientes trabajos H,y Z.

%Applications for the analysis and modeling of TS have been developed in GHZ. In the field of cloud computing and the application of techniques and algorithms for the resolution of TS, the following H and Z jobs should be considered.

%El modelado de flujo de trabajo en en la experimentación de MD/AI se considera en U,I, y O. Varias aproximaciones utiliznado lenuajes basados en otologías para la definicion de fujos de trabajo se han tratado en Z e Y. Al ser modelado de ML/AI, se consideran parte de los algoritmos que comunmente son utilizados para el análisis y modelado de ST.


%

%modeling, they are considered part of the algorithms that are commonly used for ST analysis and modeling.

%La definición de servicios genéricos de cloud computing integrando la deifinción de MD/DM se ha considerado en los trabajos T y Z. DMOP, Expoxé, MLSchema, ...

%


%Existe la necesidad de congregar las diferentes téncias y algositmos de modelado de ST, incluyendi algoritmos, Ténicas, preprocesado, Clasifiacion de Problemas, Medidas de rendimiento para los distintos tipos de TS, etc.

%Most of the proposals allow the development of complete experimental works, including part of the usual workflow with data processing and algorithms. In these works the workflow modeling with time series is not taken into account, being a fundamental element for the integration of these services within CC platforms. These types of problems need to bring together the different techniques and algorithms of ST modeling, pre-processing, performance measurements, visualization, or predictive models among others. In our work we developed a proposal of workflow modeling for time series in CC, which allows to approach the complete work with the TS experimentation. In our work we developed a proposal of workflow modeling for time series in CC, which allows to approach the complete work with the TS experimentation using Linked Data proposal  to be able to work with them from CC platforms.

%Laas herraminetas y framenwork software de modelado y anaisis de TS, han sido  utilizadas de forma satisfactoria  desde lenguajes de programaci´pn con R, python entre otros. Taskviews como el mostrado en Z.

%In recent years, software such as tools and frameworks for solving data mining and artificial intelligence problems have been developed. These tools provide a wide range of methods and algorithms for data analysis. Its capabilities include many of the most widely used methods for time series modeling, including aspects intimately related to working with ST such as preprocessing, trend studies, seasonality, etc. This set of software ranges from complete applications for workflow modeling with ST[REFs] to programming languages such as R[REF] and its taskviews for TS[REF], python[REF] among others that offer very complete libraries for working with time series modeling.

%Descripción de servicios que englobe çCC y parte de me-tdoso de TS en X.

%Description of services that includes çCCCC and part of the X-TS method.

%En nuestro trabajo se desarrolla una propuesta que concreta el flujo de rabajo con TS.

%In our work, a proposal is developed that concretizes the work flow with TS.

%Un traductor de la descirpcion del modelad de TS a implmentacion en CC ha sido desarrollado. En X e Y se realiza esto .

%A translator of the deciphering of the TS model to CC implementation has been developed. In X and Y this is done.



%%%%
%%%%
%Proveedores de cloud computing como AWS, Azure, or IBM Watson entre otros, disponen de herramientas de procesamiento masivo de datos.  Ofrecen servicios de algoritmos bajo demanda, además de herramientas de modelado de flujo de trabajo desde donde procesar problemas de MD. Multitud de trabajos han sido realizados sobre la base de utilizar la infraestructura de Cloud Computing [REFs].


==> Time Series Workflow for CC-1/timeseriesasaccservice.tex <==
\section{Time Series service description}
\label{sec:timeseries}
 
 
%%%%%
%%%%
%%%
% El modelado de Series temporales es una tarea difícil que integra diferentes operaciones, y que sigue un fujo de trabajo dinámico. En este trabajo hemos realizado un propuesta de completa para el modelado de flujo de trabajo con Series Temporales en Cloud Computing. El esquema de propuesta   se llama tswf-schema y se ha desarrollado utilizando un lenguaje semántico basado en ontologías, siguiendo las directivas de LinkedData para la definición y descripción de conceptos, entidades y relaciones con otros esquemas. Gracias a estos elementos se ha definido un esquema completo que permite modelar cualquier flujo de trabajo con series temporales, tal y como se puede observar en la sección \ref{sec:usecases}, en la que se desarrollan varios ejemplos de trabajo con Series Temporales modeladas mediante tswf-schema. El esquema está dividido en varias partes que facilitan su integración y modularidad, estas son: pre-procesamiento de los datos, visualización de los datos, funciones para el analisis de la información, trabajo con el análisis de estacionalidad, selección del modelo predictivo, clasificación del problema de aprendizaje, entrada de datos, y medidas de evaluación del rendimiento, tareas entre otras. Cada una de estas parte son desarrolladas en detalle en la parte central de esta sección.  En la figura X se puede ver el esquema general del modelado de fujo de trabajo con Serieste Temporales que se ha diseñados. Por razones de  espacio no se ha desplegado el esquema completo, dado su tamaño, por lo que se han mostrado cada uno de las clases contenedoras principales. Siguiendo la especificación de LinkedData, se ha utilizado otros vocabularios desde otros esquemas, completando y ampliando la definición del esquema. Entre los otros esquemas utilizandos se encuentan MLSchema (mls) [REFs] y skos [REFs] entre otros. 


Time Series modeling is a challenging task that integrates different actions following a dynamic \WFlong{}. In this work a complete proposal for \WFlong{} modeling with \TS{} in \CC{} has been made. The proposed  schema is called \tswfschema{}  and has been developed using a semantic language based on ontology, following the Linked Data guidelines for the definition and description of concepts, entities and relationships to other schemes. A complete diagram has been defined allowing any \WFlong{} with \TS{} to be modeled, as can be seen in the section on \ref{sec:usecases}, in which several examples of working with time series are developed and modelled using \tswfschema{} . 

The scheme is divided into several parts that facilitate its integration and modularity, these are: \textit{data pre-processing}, \textit{data visualization}, \textit{functions for information analysis}, work with \textit{seasonality analysis}, \textit{predictive model selection}, \textit{learning problem} information, \textit{data entry}, and \textit{performance evaluation measures}, among others. Each of these parts is developed in detail throughout this section. In figure \ref{fig:tswf-schema-general} you can see the general diagram of the flow rate modeling with time series that has been designed. For reasons of space, the complete scheme has not been displayed, given its size, so that each of the main container classes has been shown. Following the Linked Data specification, other vocabularies have been used from other schemes, completing and broadening the definition of the scheme.  The scheme provided by \textit{MLSchema} \cite{esteves2016ml} and \dmccschema{} \cite{parra2018data} has been used as base for the \WFlong{} of experimentation with \TS{}, in addition to other vocabularies such as \textit{SKOS} \cite{miles2009skos} or \textit{schema.org} \cite{guha2016schema} among other.



\begin{figure}[]
  \centering
   {\epsfig{file = images/tswf-schema-general, width =  \columnwidth}}
  \caption{General schema for Time Series workflow modelling}
  \label{fig:tswf-schema-general}
 \end{figure}



%%%%%
%%%%
%%
% Para la definición del modelado de flujo de trabajo se ha teniedo en cuenta un alto volumen de trabajos y libros relacionada con el modelado y analisis de series temporales. Para las clases contenedoras y otras partes que componenen el esquema, se han revisado los trabajos de investigación relacionados con el área, junto con trabajos reales de analisis de series temporales procedentes de varias fuentes [REFs]. Esto ha permitido extraer gran parte de las operaciones y métodos con los que se trabaja a la hora de hacer un modelado de series temporales. En la propuesta desarrollada en tswf-schema se ha tratado de integrar el mayor número de funcionalidades, junto con las más comunmente extendidas durante el fujo de trabajo con series temporales. Igualmente integra modelado comunmente extendido como la metodología de Box-Jenkings [REFs] así como metodologías basadas en fujo de trabajo de procesamiento de problemas de  Minería de datos junto con Machine Learning aplicado a Series Temporales.


For the definition of \WFlong{} modeling has been taken into account a high volume of research papers and books related to \TS{} modeling and analysis. For the container classes and other parts of the scheme, research related to the area has been reviewed, along with actual \TS{} analysis work from various sources such as \cite{harris2003applied} \cite{de1992some} \cite{hyndman2007automatic}. This has made it possible to extract a large part of the operations and methods used to model \TS{}, also from multiples knowledge domains. In the proposal developed in \tswfschema{} we have integrated the greatest number of functionalities, together with the most common ones during the \WFlong{} process with \TS{}. It also comprises widespread modeling such as the \textit{Box-Jenkings} \cite{tang1991time}  methodology as well as workflow-based experimentation for processing \DM{} problems and \ML{} applied to \TS{}  \cite{bontempi2012machine} \cite{ahmed2010empirical}.



%%%%%
%%%%
%%
% En cuanto a la integración de tswf-schema como servicio dentro de Cloud Computing , tswf-schema, puede ser integrado completamente con dmcc-schema [REFs]. Este esquema contienen todos los otros elementos clave en la descripción de servicios de cloud computing, tales como puntos de interacción, precios, instancias o SLA entre otros y sirve de complemento para la integración de un fujo de trabajo con Series temporales.


%As for the integration of \textit{tswf-schema} as a service within Cloud Computing , \textit{tswf-schema}, it can be fully integrated with \textit{dmcc-schema} \cite{parra2018data}. 
\textit{tswf-schema} contains all key elements in the description of cloud computing services, such as interaction points, prices, instances or SLAs, among others, and serves as a complement to the integration of a \WFlong{} with time series as a Service on \CC{} platforms. This means that it allows you to have the complete description of \CC{} services, both from a functional and a business point of view.



%%%%%
%%%%
%%
% En los siguientes párrafos, desarrollamos en detalle los componentes de la  definición de tswf-schema:

In the following subsections, all the main components of the \textit{tswf-schema} definition are detailed:


%%%%%
%%%%
%%
% Pre-procesamiento. Parte del análisis y trabajo con Series Temporales requiere de operaciones sobre los datos, donde se aplican transformaciones, reducciones, limpieza, o imputaciones entre otras. En el diagrama de la figura X se pueden ver todos los elementos más comunmente usados en el procesamiento de series temporales a nivel de datos. Básicamente se ha segmentado en varias partes, tales como Imputaciones (Imputation), Valores incoherentes (Outliers), análisis espectral,  y transformación de los datos (Scale), reducción del ruido o suavizado. Cada una de las subpartes contienen varias de las funcionalidades que se han considerado las más utilizadas en el procesamiento de estos tipos de datos, acorde con los trabajos de [REFs].

\textbf{Pre-processing.} Part of the analysis and work with \TS{} requires operations on the data, where they apply transformations, reductions, cleaning, or imputations among others. In the diagram in figure \ref{fig:tswf-schema-preprocesing} you can see all the elements most commonly used in data level time series processing. It has basically been segmented into various parts, such as imputation, \textit{outliers}, spectral analysis, scaling, noise reduction or smoothing. Each of the sub-parts contains several of the functionalities that have been considered the most commonly used in the processing of these types of data, according to the work of \cite{garcia2015data}.


\begin{figure}[]
  \centering
   {\epsfig{file = images/tswf-schema-preprocesing.png, width =  \columnwidth}}
  \caption{Preprocessing classes for Time Series workflow modelling}
  \label{fig:tswf-schema-preprocesing}
 \end{figure}


%%%%%
%%%%
%%
% Analisis de la información y Analisis de la estacionalidad. Gran parte de los estudios estadísticos con Series Temporales se basan en la metodologia Box-Jenkings, donde se aplica una serie de estudios sobre los datos de la serie temporal para comprobar la tendencia, estacionalidad entre otros, así como diferentes test estadísticos necesarios para aplicar diferentes métodos. Como se ve en la figura X, se han dividido en dos partes, por un lado el analisis de la información, que incluye test de correlacion, estacionalidad y tendencia. Por otro lado da cabida a los Test Estadísticos integrando estacionariedad, normalidad, aleatorierar, no-linealidad entre otros.

\textbf{Analysis of the information and analysis of seasonality.} Most of the statistical studies with \TS{} are based on the Box-Jenkins methodology \cite{tang1991time}, where a series of studies on the data of the time series is applied to check the trend, seasonality among others, as well as different statistical tests necessary to correctly identify the time series. As shown in figures \ref{fig:tswf-schema-informationanalysis} and \ref{fig:tswf-schema-stationalanalysis}, they have been divided into two parts, on the one hand, the analysis of the information, which includes correlation, seasonality and trend tests. On the other hand, it also includes statistical tests, integrating stationarity, normality, randomness or non-linearity among others.


\begin{figure}[]
  \centering
   {\epsfig{file = images/tswf-schema-informationanalysis.png, width = 5cm}}
  \caption{Information analysis classes for Time Series workflow modelling}
  \label{fig:tswf-schema-informationanalysis}
 \end{figure}
 
 
 \begin{figure}[]
  \centering
   {\epsfig{file = images/tswf-schema-stationalanalysis.png, width =  \columnwidth}}
  \caption{Stationary analysis classes for Time Series work-flow modelling}
  \label{fig:tswf-schema-stationalanalysis}
 \end{figure}


%%%%%
%%%%
%%
% Medidas de evaluación. La salida del flujo de trabajo de analisis de una serie temporal puede ser indentificada según el problema de estudio de Series Temporales en cuestión. Se han considerado los 4 grandes grupos de medidas, relacionadas con las más utilizadas en problemas de Series Temporales, tales como clasificación, medidas similaridad, precisión de la predicción, rendimiento del agrupamiento, o analisis de los residuos. Medidas de clasificación como F1-Score, ROC, o confusión matrix, han sito tenidas en cuenta. Para las medidas de similaridad, otras como DTW, Edit Distance o Jaccard han sido implementadas, puesto que son comunes en problemas de de este tipo. En cuanto a las medidas de Error, que identifican la calidad del ajuste de la predicción, se han incluido todas las medidas consideradas en los trabajos de [REFs]. Si el problema que se está tratando está relacionado con agrupamiento de series temporales, diferentes medidas tales como APN, AD/ADM o Silhouette W han sido tenidas en cuenta. En la figura X se detalla el conjunto de medidas de evaluación que se han incluido en tswf-schema.


\textbf{Evaluation measures.} The output of the analysis \WFlong{} of a \TS{} can be identified according to the \TS{} study problem in question. Four main groups of measures have been considered, related to those most used in \TS{} problems, such as classification, similarity measurements \cite{serra2014empirical}, precision of the forecast \cite{weigend2018time}, performance of the clustering \cite{montero2014tsclust}, or analysis of the residues. Classification measures such as \textit{F1-Score}, \textit{ROC}, or matrix confusion have been taken into account. For similarity measures, others such as \textit{DTW} \cite{mueen2016extracting}, \textit{Edit Distance} \cite{chen2015kernel} or \textit{Jaccard} \cite{aghabozorgi2015time} have been implemented, as they are common in problems of this type. As regards the \textit{Error measures}, which identify the quality of the forecast adjustment, all the measures considered in the work \cite{shcherbakov2013survey} have been included. If the problem being addressed is related to time series clustering, different measures such as \textit{APN}, \textit{AD/ADM} or \textit{Silhouette W}  have been taken into account. Figure \ref{fig:tswf-schema-evaluationmeasures} details the set of evaluation measures that have been included in \tswfschema{}.


 \begin{figure}[]
  \centering
   {\epsfig{file = images/tswf-schema-evaluationmeasures.png, width = \columnwidth}}
  \caption{Evaluation measures classes for \TS{} workflow modelling}
  \label{fig:tswf-schema-evaluationmeasures}
 \end{figure}



%%%%%
%%%%
%%
% Modelo predictivo. A la hora de instanciar un modelo que  se intente ajustar a los datos de la serie temporal, pueden aplicarse multitud de algoritmos y métodos estadísticos. En nuestro trabajo hemos integrado los algoritmos y métodos más comunmente utilizados en este área de analisis de datos sobre Series Temporales. Desde métodos estadísticos muy extendidos tales como ARIMA  o  variantes de ella (ARIMA, SARIMA, ADIMAX, ...) , además de otras como ETS entre otras. También se han implementado análisis de regresión con los métodos relacionados con Series temporales considerados en [REFs], como AR,  LASSO o MARS entre otros. Finalmente se ha considerado un parte importante de métodos procedentes del Machine Learning, principalmente procedente de estudios [REFs], estos algoritmos incluyen la aplicaión de ténicas basadas en Redes Neuronales, Random Forest o SVM entre los más destacados. El diagrama completo de los metodos y algoritmos incluidos en tswf-schema se puede ver en la figura X.

\textbf{Predictive model.} When instantiating a model that tries to fit the data of the \TS{}, a multitude of algorithms and statistical methods can be applied. In our work we have integrated the algorithms and methods most commonly used in this area of \TS{} data analysis. From widespread statistical methods such as \textit{ARIMA} or variants of it (\textit{ARIMA}, \textit{SARIMA}, \textit{ARIMAX}, etc.), as well as others such as \textit{ETS} among others. Regression analysis has also been implemented with methods related to time series considered in \cite{paolella2018linear}, such as \textit{AR}, \textit{LASSO} or \textit{MARS} among others. Finally, an important part of Machine Learning methods has been considered, mainly from \cite{de200625} studies. These algorithms include the application of techniques based on \textit{Neural Networks}, \textit{Random Forest} or \textit{SVM} among the most outstanding. The complete diagram of the methods and algorithms included in \tswfschema{} can be seen in figure \ref{fig:tswf-schema-evaluationmeasures}.

 \begin{figure}[]
  \centering
   {\epsfig{file = images/tswf-schema-predictivemodel.png, width =  \columnwidth}}
  \caption{Predictive models classes for Time Series work-flow modelling}
  \label{fig:tswf-schema-predictivemodel}
 \end{figure}



%%%%%
%%%%
%%
% Visualización de los datos. Un parte imporante de la fase de análisis dentro del trabajo sobre una serie temporal es la visualización de los datos en una serie de grafícas. Esto permite observar parte de la información visual, desde difentes tipos de trazos como despcomposicion, diferenciación o STL. En la figura X se pueden ver los implementados.


\textbf{Visualization of the data.} One part of the work is to perform repeated visualizations of the data to assess the state of the data and to use different plot analyses to better understand the shape of the data. This allows to observe some of the visual information such as decomposition, differentiation or \textit{STL} plots. Figure \ref{fig:tswf-schema-visualization} implements the set of visualizations available.


 \begin{figure}[]
  \centering
   {\epsfig{file = images/tswf-schema-visualization, width =  5cm}}
  \caption{Visualization classes for Time Series work-flow modelling}
  \label{fig:tswf-schema-visualization}
 \end{figure}


\textbf{Workflow.} The study of data generally does not follow a linear work scheme as indicated with this particular type of data, so that the data engineer or data scientist generates different flows of operations with which to compose the work during the analysis. To facilitate this task in \tswfschema{}, all operations and tasks that are performed can be composed as a linear or nonlinear sequence. If we think at a high level, this feature is what will provide the \CC{} service for \TS{} with the necessary functionality to visually compose (as building blocks) each operation or task to be performed at each time to produce a complete analysis. In figure X can be seen how this functionality intrinsic to \tswfschema{} serves to manage the flow of operations contained in the scheme.


%%%%%
%%%%
%%%
%Un factor muy imporante en la descripción de este tipo de servicios de modelado es la capacidad que poseen de ser altamente portables, es decir, una vez definido un flujo de datos completo o un simple analisis de Series temporales con tswf-schema, este es portable a cualquier plataforma de cloud computing.

==> Time Series Workflow for CC-1/usecases.tex <==
\section{Deploying Time Series services}
\label{sec:deploying}


Once all the components of \tswfschema{} have been defined in the previous section, it is necessary to present a set of examples that highlight the potential of the scheme designed to describe \TS{} workflows. 

To address the presentation of these cases, two models will be used, on the one hand a) the straightforward transcription of examples proposed in a programming language into \tswfschema{}, putting the value on the ease of translating any \TS{}-based study into a semantic agnostic model ready to be ported, deployed or executed on \CC{} providers, and b) the modelling of a cloud service with key components of the service, so that a \CC{}  service is specified and it is ready to be part of a \CC{} provider's catalogue. For the examples we will use \R{} and \python{} language, since they are one of the most extended languages and for the transcription of those example codes to the \tswfschema{} scheme we will use \jsonld{}.

In order to make the process of developing a \CC{} service based on \TS{} more comprehensible, the figure \ref{fig:cloudcomputinservice} shows the different elements that make up a \CC{} service. This figure  shows several aspects related to the definition of the service management logic, more closely linked to the definition of \CC{}, and on the other hand the description of the service functionality itself, in this case, a workflow with time series that runs as a service within a \CC{} provider's service catalogue.

\begin{figure}[]
  \centering
   {\epsfig{file = images/cloudcomputingservice.pdf, width =  0.5\columnwidth}}
  \caption{Components of a generic \CC{} service together with the functionality elements of a \TS{} service in a service catalogue.}
  \label{fig:cloudcomputinservice}
 \end{figure}
 
 

\subsection{Baseline of the structure of a \TS{} workflow}

The general minimum structure for designing and instantiating a \TS{} analysis using \tswfschema{} can be seen in the listing \ref{lst:lakehuron_skeleton}, according to the figure \ref{fig:tswf-schema-general} that outlines the overall diagram of the scheme. This skeleton contains the basic components that will be instantiated to show a functional example of the description of a workflow with \TS{}, where in line 2-3 is established which will be the context of vocabulary used for the definition in \jsonld{}, from line 6 to 10 are added the different operations of pre-processing of input data and various studies on them. Then in lines 11 and 12 are stated the methods that will be used to create the models and from line 15 the workflow information output. Each of the skeleton components is detailed in the following sections.

\footnotesize{
\begin{lstlisting}[caption={Skeleton of the component instantiation in \jsonld{}},label={lst:lakehuron_skeleton},language=json,firstnumber=1]
{
 "@context": {
    "tswf": "http://dicits.ugr.es/linkeddata/tswf-schema/"
  },
  ...
  "tswf:hasInput": {
    "tswf:hasPlot": {...},
    "tswf:hasInformationAnalysis": {...},
    "tswf:hasStationaryAnalysis": {...}
   },
  "tswf:performs": {
    "tswf:hasTSAnalysis": {...},
    ...
    }
  "tswf:hasOutput": {
  
  },
  ...
 }
\end{lstlisting}
}

\subsection{A model of \TS{} analysis}

For this use case we will use an example of an actual time series analysis, implemented in the \R{} language. This example consists of a series of basic steps that reproduce the modeling of a simple \TS{} example. This workflow can be seen visually in the figure \ref{fig:lakehuronhighleveloperative}.

\begin{figure}[]
  \centering
   {\epsfig{file = images/LakeHuronHighLevelOperative.jpg, width =  \columnwidth}}
  \caption{Diagram of the operations and tasks carried out for the case study use of Lake Huron.}
  \label{fig:lakehuronhighleveloperative}
 \end{figure}

The full code in \R{} and \python{} of the workflow implementation can be found in the scheme repository \cite{RepoDicitsTSWF}. In the description of the use case, we represent some parts of the modeling as a service, so we can compare the \R{}-language code transcription to the \tswfschema{} scheme with \jsonld{} as a semantic description language. This is not to replace one language with another, but with \tswfschema{} a complete description of a high level workflow is provided, abstracting the programming support, the platform or the computing environment. One of the advantages of using semantic models is that you can indicate the level of detail you want in each defined aspect. This is more expressive and less complex to understand, leaving more core aspects to the implementation of the underlying system that manages the schema, such as the default settings.

\begin{figure}[]
  \centering
   {\epsfig{file = images/simpletswf.pdf, width = \columnwidth}}
  \caption{Diagram of the components and operations of a simple TS analysis use case using \tswfschema{}.}
  \label{fig:lakehurontswf}
 \end{figure}
 
 One of the advantages of using semantic description technologies to define services or functions is that you can indicate the level of detail you want in each defined aspect. This is more expressive and less complex to understand, leaving more core aspects to the implementation of the underlying system that manages the schema, such as the default settings.

\subsubsection{\TS{} Analysis: Workflow information and description}

The definition of services in general terms requires a minimum of basic information describing what is being implemented. In our case, the first step to define the workflow instantiation with \tswfschema{} is the description of the analysis, through the main class \texttt{TSAnalysis}.With \texttt{TSAnalysis} and its properties all the attributes considered key in the definition of what is going to be deployed are declared so that it can be described in the most efficient way possible and with a friction-less integration in catalogs or marketplace of services in Cloud Computing. Aspects related to the automatic discovery of services for \CC{} would be defined from this class. For space reasons not all attributes of \texttt{TSAnalysis} will be exposed, so only some basic ones are shown in the listing \ref{lst:lakehuron_TSAnalysis}.

\footnotesize{
\begin{lstlisting}[caption={Definition of the basic information of time series analysis.},label={lst:lakehuron_TSAnalysis},language=json,firstnumber=1]
"@context": {
    "tswf": "http://dicits.ugr.es/linkeddata/tswf-schema/"
  },
  "@id": "http://dicits.ugr.es/tswf-marketplace/#TS_eb09t74",
  "@type": "tswf:TSAnalysis",
  "tswf:name": "TS Analysis base with code TS_eb09t74",
  "tswf:description": "This is an example of TS an.",
  "tswf:author": "This is an example of TS an.",
  "tswf:dateCreated": "2020-09-01 10:30:00",
  "tswf:version": "Test version 1.0",
  "tswf:codeRepository": {
        "@type":"tswf:url",
        "@value":"https://"
        } 
  "tswf:hasInput": ...
\end{lstlisting}
}

In the first lines (lines 1 to 3) the context of the overall \texttt{TSAnalysis} description is declared in which \tswfschema{} will be used. The context allows applications to use a set of terms to communicate with one another more efficiently, but without losing accuracy. Then, each instance of \texttt{TSAnalysis} created with \tswfschema{} must be marked with an identifier that uniquely relates this workflow, for example, within a particular catalog, for which \texttt{@id} is specified (line 4). The \texttt{@type} property indicates that all the remaining content corresponds to a \texttt{TSAnalisys} and subsequently part of its attributes are declared (lines from 5 to 13), such as the \TS{} name, description of the workflow, or the repository where the code of the described service will be hosted, to take the description of the flow to execute it (lines 11-14). The rest of the properties of the workflow components are instantiated in the following subsections (from line 15, with "\texttt{tswf:hasInput}", "\texttt{tswf:hasOutput}", etc. as described within  figure X). 

%


\subsubsection{Data input}

To perform the ingestion of the data of a time series, basically in the \R{} language the data can be loaded from different sources, such as \textit{CSV} format for example. In \CC{} environments or other computing platforms it is possible that data can come from databases, \TS{} databases, or even data steaming services.  In this way,  just as \R{} or \python{} supports data ingest from multiple sources, \tswfschema{} has the possibility to include very diverse data sources. For the data input instantiating it is necessary to at least define the data source, the source type and the fields that will be used during the whole analysis process. In the listing \ref{lst:lakehuron_hasInput}, a simple instantiation of the data entry is shown, where over the line number \texttt{2} is indicated the type of entry (\texttt{tswf:Data}), the type of source (\texttt{tswf:CSVFile}  in this case) in lines \texttt{3-4} and where physically are the data by means of the property \texttt{tswf:src} (line 5). Then, with \texttt{tswf:fields} the features and fields of the data source are set within the lines \texttt{6-12}. 



\footnotesize{
\begin{lstlisting}[caption={Instantiation of the data entry source and its parameterization.},label={lst:lakehuron_hasInput},language=json,firstnumber=1]
...
"tswf:hasInput": {
  "@type": "tswf:Data",
  "tswf:source": {
    "@type": "tswf:CSVFile",
    "tswf:src": "///dicits/examples/lakehuron.csv",
    "tswf:fields": {
       "@set": [
         {"@value": "Year",
          "@type": "tswf:datetime"},
         {"@value": "Level",
          "@type": "tswf:integer"}
        ]
      }
    },
    ...
\end{lstlisting}
}
The transformation of the initial data intake part into \tswfschema{} is done at a higher level, since semantically each operation is labeled with its properties. This allows not having to define in advance each detail of the parameterization (or indeed the application of the \TS{} type), so that this complexity can be left to the underlying system or platform as the service responsible for making these tweaks. 

\subsubsection{Preliminary exploratory analysis}

A basic part of the analysis of \TS{} data is exploratory data analysis where the data can be plotted, checked for patterns or trends, verified for seasonality or the presence of cycles, among others. In the example, we are dealing with, through the input data we make several key charts to visually understand the problem. We consider for instance \pacf{} (\textit{Partial Autocorrelation Function}), \acf{} (\textit{Autocorrelation Function}), \stl{} (Seasonal and Trend decomposition using \textit{Loess}) as well as a visual representation of the data. 

The graphical representation of the input data is done from the \texttt{tswf:hasPlot} property. In \tswfschema{} there is a set of possible definitions of the most commonly used diagrams and charts within \TS{} analysis, so to instantiate a type of chart that you want to display is only needed to include the list of types that are required for the analysis as shown in listing \ref{lst:lakehuron_hasPlot}. Note that the level of detail selected to instantiate these types of chars does not include parameterization except in \texttt{tswf:PlotPACF}, this is because the internal implementation will be in charge of using the correct visualization with the default parameters of each chart type for the input data. On the other hand, for \texttt{tswf:PlotPACF} a \texttt{lag} parameter (\texttt{tswf:parameters}) and its specific value have been indicated (lines from 6 to 12). 


\footnotesize{
\begin{lstlisting}[caption={Set of diagrams/charts that are deployed},label={lst:lakehuron_hasPlot},language=json,firstnumber=1]
...
"tswf:hasPlot":{
      "@type": "tswf:TSPlot",
      "@set":[
        {"@type":"tswf:PlotSTL"},
        {"@type":"tswf:PlotACF"},
        {"@type": "tswf:PlotPACF",
          "tswf:parameters": {
            "@set": [
              {"tswf:name":"lag", "@value": 10}
            ]
          }
        },
        {"@type":"tswf:PlotRegular"}
      ]
    },
    ...
\end{lstlisting}
}





\footnotesize{
\begin{lstlisting}[caption={\TS{} information analysis.},label={lst:lakehuron_hasInformationAnalysis},language=json,firstnumber=1]
...
"tswf:hasInformationAnalysis": {
      "@type": "tswf:InformationAnalysis",
      "@set": [
        {"@type": "tswf:LagStudy"},
        {"@type": "tswf:TrendSTL"},
        {"@type": "tswf:ACF"},
        {"@type": "tswf:PACF"}
      ]
    },
    ...
\end{lstlisting}
}


Further on, in the listings \ref{lst:lakehuron_hasInformationAnalysis} and \ref{lst:lakehuron_hasStationaryAnalysis} are shown how it is possible to add  different studies used in the analysis, such as \textit{Information Analysis}, or \textit{Stationary Analysis}. For both types of studies, following the scheme shown in figures \ref{fig:tswf-schema-informationanalysis} and \ref{fig:tswf-schema-stationalanalysis}, it is possible to include their corresponding tests and operations. For the analysis of the information, as shown in list \ref{lst:lakehuron_hasInformationAnalysis}, four basic studies have been added in the work with \TS{} (lines 4 to 8).  In the same way as with the descriptions of the charts, we have taken all the default parameters for this example. On the other hand, in the study of stationarity analysis shown in list \ref{lst:lakehuron_hasStationaryAnalysis} four basic tests have been added (lines 4 to 8).

\footnotesize{
\begin{lstlisting}[caption={\TS{} stationary analysis.},label={lst:lakehuron_hasStationaryAnalysis},language=json,firstnumber=1]
...
"tswf:hasStationaryAnalysis": {
      "@type": "tswf:StatitionaryAnalysis",
      "@set": [
        {"@type": "tswf:StatisticalTest"},
        {"@type": "tswf:DickeyFuller"},
        {"@type": "tswf:JarqueBera"},
        {"@type": "tswf:JungBox"}
      ]
    },
    ...
\end{lstlisting}
}


\subsubsection{Predictive model and evaluation measures}

Once the exploratory analysis is done, the selection and adjustment of the model is performed. The selection of the best model depends on the availability of historical data or the dependence of variables. Hence it is often necessary to compare several predictive models to see how the data actually behave. For this example the \R{} code of the three models displayed in listing \ref{fig:lakehuronhighleveloperative}, where an \texttt{AR} regression model, an \ARIMA{} modeling and finally an \SVM{} algorithm are used. The consequent code in the \tswfschema{} scheme corresponds to the listing  code \ref{fig:lakehuronhighleveloperative}. For each of the methods,  it is possible to specify the parameterization, in this case only for the \ARIMA{} model has been specified. In listing \ref{lst:lakehuron_performs}, from line 2 to line 5, a model based on Machine Learning functions/operations is specified, such as \texttt{SVM} (\texttt{tswf:SVM}). Another regression-based model is indicated in lines 10-12 (\texttt{tswf:AR}) and finally, with \texttt{tswf:ARIMA} (lines 7-15) an \texttt{ARIMA} model is instantiated, with a partial parameterization (\texttt{tswf:parameters}) as it appears in lines 11-13 including \texttt{order}, \texttt{seasonal} and \texttt{lambda}.




\footnotesize{
\begin{lstlisting}[caption={\TS{} predictive model.},label={lst:lakehuron_performs},language=json,firstnumber=1]
...
"tswf:performs": {
      "@type": "tswf:PredictiveModel",
      "tswf:hasMLAnalysis": {
        "@type": "tswf:SVM"
      },
      "tswf:hasTSAnalysis": {
        "@type": "tswf:ARIMA",
        "tswf:parameters": {
          "@set": [
            {"tswf:name": "order", "@value": [0,0,1])},
            {"tswf:name": "seasonal", "@value": [0,0,1])},
            {"tswf:name": "lambda", "@value": 0)}
          ]
        }
      },
      "tswf:hasTSRegression": {
        "@type": "tswf:AR"
      }
    },
...
\end{lstlisting}
}

Finally, as part of the explicit output of the workflow, using the \texttt{tswf:hasOutput} property, it is possible to indicate what kind of additional information can be analyzed as a result of the full process (listing \ref{ls:lakehuron_evaluationmeasures}, line 2). This has included in the output of the workflow the prediction function, which is called to return the results on how is the forecasting on different horizons, by giving the user of different measures to evaluate the performance of the forecasts, for example (see figure \ref{fig:tswf-schema-evaluationmeasures}). In the listing  \ref{ls:lakehuron_evaluationmeasures}, lines 5-10 we have chosen to include two measures (RMSE and MSE) for the evaluation (\texttt{tswf:EvaluationMeasures}) with which you can verify the accuracy of the forecast (\texttt{tswf:ForecastAccuracy}), made with the models generated in the previous stage through the property \texttt{tswf:performs} (in this instance \texttt{AR}, \texttt{ARIMA} and \texttt{SVN}).

\footnotesize{
\begin{lstlisting}[caption={\TS{} evaluation measures.},label={lst:lakehuron_evaluationmeasures},language=json,firstnumber=1]
...
 "tswf:hasOutput": {
      "@type": "tswf:EvaluationMeasures",
      "@set": [
        {
          "id": "tswf:TSFCastAccu",
          "@type": "tswf:ForecastAccuracy",
          "tswf:hasMeasures": [
            {"@type": "tswf:RMSE"},
            {"@type": "tswf:MSE"}
          ]
        }
      ]
    }
...
\end{lstlisting}
}





\subsection{A \CC{} service for \TS{}}
\label{subsec:ccserviceforts}

The \TS{} example provided in the section \ref{sec:timeseries} is defining a workflow as if we were doing it in a programming language like R or Python, but using \jsonld{} as a description language. With \tswfschema{} it is possible to package \TS{} workflows and make them portable between different computing platforms by reading the description and operating each high-level component on an underlying platform or by using a \textit{Broker} to decide which \textit{SVM} or \textit{ARIMA} implementation at the low-level will be used to process a particular element. This gives an idea of the potential of using this type of semantic technology to tackle the deployment of services in \CC{}. In this manner for this use case we want to put the value how \texttt{tswf-schema} can be integrated to support a \CC{} service for \TS{}. 

Following the principles of \textit{Linked Data} for semantic data, we will reuse another scheme called \texttt{dmcc-schema} \cite{parra2020semantics} that allows unifying all the basic aspects of the definition and management of a \CC{} service including costs/prices, catalog or \textit{SLA} among others, together with the functionality such as a \TS{} analysis.

   \begin{figure}[ht]
    \centering
    \begin{pgfpicture}
        \pgftext{\pgfimage[width=\columnwidth,height=5cm]{dmcc+tswfcc.png}}
        \label{fig:DMCCTSWF}
    \end{pgfpicture}
    \end{figure}

In figure \ref{fig:DMCCTSWF} a diagram can be seen combining both schemes to complete the description of a \TS{} workflow with the management of a \CC{} service.





==> Time Series Workflow for CC-1/validation.tex <==
\section{Validation}

%Ademas de ofrecer en la seccion anterior un conjunto de ejemplos completos de modelado de TS utilizando el esquema, para afianzar la validez de TSWF como mecanismo para la definicion de servicios de analisis de TS, hemos llevado a cabo tres acciones adcionales de validacion, tales como MarketPlace de servicios de TS para CC con TSWF, preguntas de competecia, e integración en un escenario práctico.

%- Competence questions: Creacion de una serie de CQ con el objetivo de testear si TSWF se ajusta correctamente al domino del problema y es capaz de resolver de forma precisa las consultas que se le realizan. Con estas CQs se intenta cubrir una parte importante de la definicion de un servicio TS en CC, considerando los elementos clave, como el estudio, analisis, o modelos predictivos y tambien la gestion del propio flujo de trabajo de la TS dentro del proveedor de CC (gestion del servicio). La CQs seleccionadas son las siguientes: 

In addition to giving in the previous section of examples of \TS{} modeling using \tswfschema{}, to reinforce the validity of the scheme as a mechanism for the definition of \TS{} analysis services in \CC{}, we have carried out two additional validation actions, such as \marketplace{} of \TS{} services for \CC{} with \tswfschema{} and a set of competence questions (\CQs{}) . 


\subsection{\TS{} \marketplace{}}  

% Al trabajar con definiciones y descripciones semánticas una prueba de validez de la tecnología a efectos prácticos consiste en desplegar esos componentes de manera efectiva dentro catálogos de descripciones. Estos catálogos tienen una doble utilidad, por un lado servir como repositorio de definiciones de servicios y por otro lado ofrecer un punto de descubrimiento de servicios por parte de entidades programáticas capaces de comprender los mismos. Un ejemplo de catálogo de servicios con descripciones que pueden ser importadas, intercambiadas,  descubiertas y consumidas ha sido diseñado como parte de un  MarketPlace de Series Temporales. El diseño del MarketPlace contiene 3 aspectos básicos: importación, composición y consumo de servicios de Time Series:

Dealing with semantic definitions and descriptions, a test of the validity of the technology for practical purposes is to deploy these components effectively within service catalogs. These catalogs have a twofold function, on the one hand, to serve as a repository of service definitions and on the other hand to provide a point of service discovery by programmatic entities having the ability to understand the services exposed. An example of a service catalog with descriptions that can be imported, exchanged, discovered, and consumed has been designed as part of a \TS{} \marketplace{}. The design of this  \marketplace{} contains 3 key features:

\begin{itemize}
    \item \textbf{Import}, where the platform allows users to include their own \tswfschema{}
    instances in \jsonld{} or \textit{\ttl{}} format. With this tool, service descriptions are
    validated and included in the catalog. Once in the catalog, it is possible to use the composition tool where the workflow description can be modeled or viewed using the \tswfschema{} elements in a visual way. Figure \ref{fig:importflow} shows the workflow import diagram to the \TS{} \marketplace{} and a part of the service catalog of available \TS{} containing all the basic attributes and details deployed. For each \TS{} it is possible to explore the definition and the components that integrate it, as well as the possibility to share/download each service available in the catalog.
    
    \begin{figure}[ht]
    \centering
    \begin{pgfpicture}
        \pgftext{\pgfimage[width=\columnwidth,height=5cm]{importflow.png}}
        \label{fig:importflow}
    \end{pgfpicture}
    \end{figure}
    
   \item \textbf{Composition},  similar to other platforms, composition offers a complementary visual tool for creating/modifying \TS{} workflows and services. In this sense it makes it much easier to compose workflows in general, since visually it is much more comfortable to use a visual tool than to code it manually. An example of the platform showing a workflow with example \TS{} is shown in the Figure \ref{fig:composeflow}. In this figure a set of  workflow operations that the service is capable of deploying are depicted. 
   
   \begin{figure}[ht]
    \centering
    \begin{pgfpicture}
        \pgftext{\pgfimage[width=\columnwidth,height=5cm]{composeflow.png}}
        \label{fig:composeflow}
    \end{pgfpicture}
    \end{figure}
    
    
    \item  \textbf{Service consumption}, once the descriptions of \tswfschema{} instances are published, they are available for consumption either manually or automatically, for example, to deploy them from \CC{} providers.
\end{itemize}

The platform is available for use in production in the website of the project \cite{noauthor_datamining-ld_nodate} and the source code is available in a \textit{Github}  repository \cite{noauthor_dicits/tswf-marketplace_2020}, in this way it is possible to deploy the \TS{} \marketplace{} in any other provider of \CC{} services. 




%-Importación: La plataforma permite a los usuarios incluir sus propios TSWFs en formato JSONLD o TTL. Con esta herramienta se validan las descripciones de los servicios y se incluyen en el catálogo. Una vez en el catálogo ya es posible utilizar la herramienta de composición donde visualmente la descripción sea modelada utilizando los elementos de tswf-schema.
%-Composición: De modo similar a otras plataformas, la composición ofrece una herramienta complementaria para crear/modificar flujos de trabajo y servicios de TS.
%-Consumo de servicios: Una vez publicadas las descripciones, éstas ya están disponibles para su consumo de forma manual o automática, por ejemplo para ejecutarlas desde servicios de computación de proveedores de Cloud Computing.


\subsection{Competency Questions (CQs)} 
Competency questions (CQs)~\cite{uschold1996} are used to specify the knowledge that has to be entailed in the ontology/vocabulary and thus can be considered to be requirements on the content of the ontology.
A way to validate a semantic schema is the creation of a series of \CQs{} to test whether the \tswfschema{} correctly fits the problem domain and is able to accurately solve the queries made to it. With these \CQs{} we try to cover an important part of the definition of a \TS{} service in \CC{} , considering key elements such as, the study, analysis, or predictive models and also the management of the workflow of the \TS{} itself within the \CC{} provider (aspects like \CC{} service management is shown in section \ref{subsec:ccserviceforts}). The selected 10 \CQs{} are the following: 

\begin{description}
\item [CQ01] \textit{How many operations [tasks] does the X \TS{} workflow for predictive analysis have?}\\Response: .

\item [CQ02] \textit{What services from the catalog [of a \CC{} provider] enable the use of \TS{} processing functions?}\\Response: .

\item [CQ03] \textit{Does the \TS{} service provide algorithms [functions] for predictive analysis using Deep Neural Networks and does it provide an SVM algorithm?}\\Response: .


\item [CQ04] \textit{What data input does the \TS{} workflow need with the X-identifier?}\\Response: .

\item [CQ05] \textit{What are the outputs of the X-identifier of a \TS{} workflow for the \CC{} service?}\\Response: .

\item [CQ06] \textit{What is the estimated economic cost of running a \TS{} workflow analysis for the \CC{}  provider X?
}\\Response: .

\item [CQ07] \textit{Is there authentication for the execution of the \TS{} service for provider X?}\\Response: .

\item [CQ08] \textit{What is the parameterization of the ARIMA algorithm?}\\Response: .

\item [CQ09] \textit{Can you display the prediction data for a horizon of X days for the Y workflow?}\\Response: .

\item [CQ10] \textit{Which predictive model of the analysis produces the results with the lowest RMSE error?}\\Response: .


\end{description}


The aim is to confirm that with \tswfschema{} is possible to capture  partially the  features  of a specific \TS{} service and it can be integrated into a service definition, through which make queries and manage this type of services for multiple \CC{} providers. Dataset, \CQs{} and \textit{SparQL} queries (endpoint) are available on the project website \cite{noauthor_datamining-ld_nodate}.


